Maximum waiting time in heavy-tailed fork-join queues

In this paper, we study the maximum waiting time $\max_{i\leq N}W_i(\cdot)$ in an $N$-server fork-join queue with heavy-tailed services as $N\to\infty$. The service times are the product of two random variables. One random variable has a regularly varying tail probability and is the same among all $N$ servers, and one random variable is Weibull distributed and is independent and identically distributed among all servers. This setup has the physical interpretation that if a job has a large size, then all the subtasks have large sizes, with some variability described by the Weibull-distributed part. We prove that after a temporal and spatial scaling, the maximum waiting time process converges in $D[0,T]$ to the supremum of an extremal process with negative drift. The temporal and spatial scaling are of order $\tilde{L}(b_N)b_N^{\frac{\beta}{(\beta-1)}}$, where $\beta$ is the shape parameter in the regularly varying distribution, $\tilde{L}(x)$ is a slowly varying function, and $(b_N,N\geq 1)$ is a sequence for which holds that $\max_{i\leq N}A_i/b_N\overset{\mathbb{P}}{\longrightarrow}1$, as $N\to\infty$, where $A_i$ are i.i.d.\ Weibull-distributed random variables. Finally, we prove steady-state convergence.

==> refs.tex <==
@book{borodin2015handbook,
  title={Handbook of Brownian motion-facts and formulae},
  author={Borodin, Andrei N and Salminen, Paavo},
  year={2015},
  publisher={Springer Science \& Business Media}
}




@article{scholMOR,
author = {Schol, Dennis and Vlasiou, Maria and Zwart, Bert},
title = {Large Fork-Join Queues with Nearly Deterministic Arrival and Service Times},
journal = {Mathematics of Operations Research},
doi = {10.1287/moor.2021.1171},
  volume={47},
  number={2},
  pages={1335--1364},
  year={2021},
  publisher={INFORMS}
}


@book{embrechts2013modelling,
  title={Modelling extremal events: for insurance and finance},
  author={Embrechts, Paul and Kl{\"u}ppelberg, Claudia and Mikosch, Thomas},
  volume={33},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@book{de2007extreme,
  title={Extreme value theory: an introduction},
  author={{\VAN{Haan}{de}{de}} Haan, Laurens and Ferreira, Ana},
  year={2006},
  publisher={Springer Science \& Business Media}
}

@article{MeijerSchol2021,
  title={{Extreme-value theory for large fork-join queues, with applications to high-tech supply chains}},
  author={Meijer, Mirjam and Schol, Dennis and {\VAN{Jaarsveld}{van}{van}} Jaarsveld, Willem and Vlasiou, Maria and Zwart, Bert},
  journal={https://arxiv.org/abs/2105.09189},
  volume={},
  number={},
  pages={},
  year={2021}
}

@article{altendorfer2011,
  title={Simultaneous optimization of capacity and planned lead time in a two-stage production system with different customer due dates},
  author={Altendorfer, Klaus and Minner, Stefan},
  journal={European Journal of Operational Research},
  volume={213},
  number={1},
  pages={134--146},
  year={2011},
  publisher={Elsevier}
}
@article{asmussen1995,
  title={{Discretization error in simulation of one-dimensional reflecting Brownian motion}},
  author={Asmussen, S{\o}ren and Glynn, Peter W and Pitman, Jim},
  journal={The Annals of Applied Probability},
  pages={875--896},
  year={1995},
  publisher={JSTOR}
}


@book{asmussen2003applied,
  title={Applied probability and queues},
  author={Asmussen, S{\o}ren},
  volume={2},
  year={2003},
  publisher={Springer}
}


@article{bernstein2006,
  title={Inventory policies in a decentralized assembly system},
  author={Bernstein, Fernando and DeCroix, Gregory A},
  journal={Operations Research},
  volume={54},
  number={2},
  pages={324--336},
  year={2006},
  publisher={INFORMS}
}
@article{bollapragada2004,
  title={Managing inventory and supply performance in assembly systems with random supply capacity and demand},
  author={Bollapragada, Ramesh and Rao, Uday S and Zhang, Jun},
  journal={Management Science},
  volume={50},
  number={12},
  pages={1729--1743},
  year={2004},
  publisher={INFORMS}
}
@article{bradley2002,
  title={Managing capacity and inventory jointly in manufacturing systems},
  author={Bradley, James R and Glynn, Peter W},
  journal={Management Science},
  volume={48},
  number={2},
  pages={273--288},
  year={2002},
  publisher={INFORMS}
}
@article{masih2011,
  title={A single-period analysis of a two-echelon inventory system with dependent supply uncertainty},
  author={Masih-Tehrani, Behdad and Xu, Susan H and Kumara, Soundar and Li, Haijun},
  journal={Transportation Research Part B: Methodological},
  volume={45},
  number={8},
  pages={1128--1151},
  year={2011},
  publisher={Elsevier}
}
@article{mayorga2011,
  title={Joint management of capacity and inventory in make-to-stock production systems with multi-class demand},
  author={Mayorga, Maria E and Ahn, Hyun-Soo},
  journal={European Journal of Operational Research},
  volume={212},
  number={2},
  pages={312--324},
  year={2011},
  publisher={Elsevier}
}
@article{pan2016,
  title={Component procurement strategies in decentralized assembly systems under supply uncertainty},
  author={Pan, Wenting and So, Kut C},
  journal={IIE Transactions},
  volume={48},
  number={3},
  pages={267--282},
  year={2016},
  publisher={Taylor \& Francis}
}
@article{reddy2020,
  title={Capacity investment and inventory planning for a hybrid manufacturing-remanufacturing system in the circular economy},
  author={Reddy, K Nageswara and Kumar, Akhilesh},
  journal={International Journal of Production Research},
  pages={1--29},
  year={2020},
  publisher={Taylor \& Francis}
}
@article{reed2017,
  title={Managing capacity and inventory jointly for multi-server make-to-stock queues},
  author={Reed, Josh and Zhang, Bo},
  journal={Queueing Systems},
  volume={86},
  number={1--2},
  pages={61--94},
  year={2017},
  publisher={Springer}
}
@article{sleptchenko2003,
  title={Trade-off between inventory and repair capacity in spare part networks},
  author={Sleptchenko, Andrei and van der Heijden, Matthijs C and van Harten, Aart},
  journal={Journal of the Operational Research Society},
  volume={54},
  number={3},
  pages={263--272},
  year={2003},
  publisher={Taylor \& Francis}
}
@article{svoboda2020,
  title={Typology and literature review on multiple supplier inventory control models},
  author={Svoboda, Josef and Minner, Stefan and Yao, Man},
  journal={European Journal of Operational Research},
  year={2020},
  publisher={Elsevier}
}
@article{wu2014,
  title={{Optimal control of a Brownian production/inventory system with average cost criterion}},
  author={Wu, Jingchen and Chao, Xiuli},
  journal={Mathematics of Operations Research},
  volume={39},
  number={1},
  pages={163--189},
  year={2014},
  publisher={INFORMS}
}
@article{zou2004,
  title={Channel coordination in an assembly system facing uncertain demand with synchronized processing time and delivery quantity},
  author={Zou, X and Pokharel, S and Piplani, R},
  journal={International Journal of Production Research},
  volume={42},
  number={22},
  pages={4673--4689},
  year={2004},
  publisher={Taylor \& Francis}
}
@book{harrison2013, 
    place={Cambridge}, 
    title={Brownian Models of Performance and Control}, 
    DOI={10.1017/CBO9781139087698}, 
    publisher={Cambridge University Press}, 
    author={Harrison, J Michael}, 
    year={2013}
}

@book{beirlant2004statistics,
  title={Statistics of extremes: theory and applications},
  author={Beirlant, Jan and Goegebeur, Yuri and Segers, Johan and Teugels, Jozef L},
  volume={558},
  year={2004},
  publisher={John Wiley \& Sons}
}
@book{leadbetter2012extremes,
  title={Extremes and related properties of random sequences and processes},
  author={Leadbetter, Malcolm R and Lindgren, Georg and Rootz{\'e}n, Holger},
  year={1983},
  publisher={Springer Science \& Business Media}
}

@book{resnick2013extreme,
  title={Extreme values, regular variation and point processes},
  author={Resnick, Sidney I},
  year={1987},
  publisher={Springer}
}

@article{berman1962limiting,
  title={Limiting distribution of the maximum term in sequences of dependent random variables},
  author={Berman, Simeon M},
  journal={The Annals of Mathematical Statistics},
  volume={33},
  number={3},
  pages={894--908},
  year={1962},
  publisher={JSTOR}
}
@article{halfin1981heavy,
  title={Heavy-traffic limits for queues with many exponential servers},
  author={Halfin, Shlomo and Whitt, Ward},
  journal={Operations Research},
  volume={29},
  number={3},
  pages={567--588},
  year={1981},
  publisher={Informs}
}

@book{vaart_1998, 
place={Cambridge}, 
series={Cambridge Series in Statistical and Probabilistic Mathematics}, 
title={Asymptotic Statistics}, 
DOI={10.1017/CBO9780511802256}, 
publisher={Cambridge University Press}, 
author={{\VAN{Vaart}{van der}{van der}} Vaart, Aad W}, 
year={1998}, 
collection={Cambridge Series in Statistical and Probabilistic Mathematics}}

@article{zielinski2009,
  title={{Optimal nonparametric quantile estimators. Towards a general theory. A survey}},
  author={Zieli{\'n}ski, Ryszard},
  journal={Communications in Statistics-Theory and Methods},
  volume={38},
  number={7},
  pages={980--992},
  year={2009},
  publisher={Taylor \& Francis}
}

@article{debicki2020exact,
  title={{Exact asymptotics of component-wise extrema of two-dimensional Brownian motion}},
  author={D\k{e}bicki, Krzysztof and Ji, Lanpeng and Rolski, Tomasz},
  journal={Extremes},
  volume={23},
  number={},
  pages={569-–602},
  year={2020}
}

@article{kou2016first,
  title={{First-passage times of two-dimensional Brownian motion}},
  author={Kou, Steven and Zhong, Haowen and others},
  journal={Advances in Applied Probability},
  volume={48},
  number={4},
  pages={1045--1060},
  year={2016},
  publisher={Applied Probability Trust}
}

@article{debicki2015extremes,
  title={{Extremes of vector-valued Gaussian processes: Exact asymptotics}},
  author={D\k{e}bicki, Krzysztof and Hashorva, Enkelejd and Ji, Lanpeng and Tabi{\'s}, Kamil},
  journal={Stochastic Processes and their Applications},
  volume={125},
  number={11},
  pages={4039--4065},
  year={2015},
  publisher={Elsevier}
}




@article{flatto1984two,
  title={{Two parallel queues created by arrivals with two demands I}},
  author={Flatto, Leopold and Hahn, Sann},
  journal={SIAM Journal on Applied Mathematics},
  volume={44},
  number={5},
  pages={1041--1053},
  year={1984},
  publisher={SIAM}
}
@article{flatto1985two,
  title={{Two parallel queues created by arrivals with two demands II}},
  author={Flatto, Leopold},
  journal={SIAM Journal on Applied Mathematics},
  volume={45},
  number={5},
  pages={861--878},
  year={1985},
  publisher={SIAM}
}

@article{wright1992two,
  title={Two parallel processors with coupled inputs},
  author={Wright, Paul E},
  journal={Advances in Applied Probability},
  volume={24},
  number={4},
  pages={986--1007},
  year={1992},
  publisher={Cambridge University Press}
}

@article{baccelli1985two,
  title={{Two parallel queues created by arrivals with two demands: The $M/G/2$ symmetrical case}},
  author={Baccelli, Fran{\c{c}}ois},
  year={1985},
  journal={Technical report RR--0426, INRIA}
}

@phdthesis{de1988fredholm,
  title={Fredholm integral equations in queueing analysis},
  author={Klein, Stephanus J de},
  year={1988},
  school={Rijksuniversiteit Utrecht}
}

@article{ko2004response,
  title={{Response times in $M/M/s$ fork-join networks}},
  author={Ko, Sung-Seok and Serfozo, Richard F.},
  journal={Advances in Applied Probability},
  volume={36},
  number={3},
  pages={854--871},
  year={2004},
  publisher={Cambridge University Press}
}

@article{ko2008sojourn,
  title={{Sojourn times in $G/M/1$ fork-join networks}},
  author={Ko, Sung-Seok and Serfozo, Richard F},
  journal={Naval Research Logistics (NRL)},
  volume={55},
  number={5},
  pages={432--443},
  year={2008},
  publisher={Wiley Online Library}
}

@article{knessl1991diffusion,
  title={On the diffusion approximation to a fork and join queueing model},
  author={Knessl, Charles},
  journal={SIAM Journal on Applied Mathematics},
  volume={51},
  number={1},
  pages={160--171},
  year={1991},
  publisher={SIAM}
}

@article{baccelli1989queueing,
  title={Queueing models for systems with synchronization constraints},
  author={Baccelli, Fran{\c{c}}ois and Makowski, Armand M},
  journal={Proceedings of the IEEE},
  volume={77},
  number={1},
  pages={138--161},
  year={1989},
  publisher={IEEE}
}

@article{nelson1988approximate,
  title={Approximate analysis of fork/join synchronization in parallel queues},
  author={Nelson, Randolph and Tantawi, Asser N},
  journal={IEEE Transactions on Computers},
  volume={37},
  number={6},
  pages={739--743},
  year={1988},
  publisher={IEEE}
}

@book{nelson1987approximating,
  title={Approximating task response times in fork/join queues},
  author={Nelson, Randolph and Tantawi, Asser N},
  year={1987},
  publisher={IBM Thomas J. Watson Research Division}
}



@article{brown1977extreme,
  title={Extreme values of independent stochastic processes},
  author={Brown, Bruce M and Resnick, Sidney I},
  journal={Journal of Applied Probability},
  pages={732--739},
  year={1977},
  publisher={JSTOR}
}


@article{dieker2005extremes,
  title={{Extremes of Gaussian processes over an infinite horizon}},
  author={Dieker, AB},
  journal={Stochastic processes and their applications},
  volume={115},
  number={2},
  pages={207--248},
  year={2005},
  publisher={Elsevier}
}


@article{asmussen1982conditioned,
  title={{Conditioned limit theorems relating a random walk to its associate, with applications to risk reserve processes and the $GI/G/1$ queue}},
  author={Asmussen, S{\o}ren},
  journal={Advances in Applied Probability},
  pages={143--170},
  year={1982},
  publisher={JSTOR}
}

@phdthesis{varma1990heavy,
  title={Heavy and light traffic approximations for queues with synchronization constraints},
  author={Varma, Subir},
  year={1990},
  school={University of Maryland}
}

@article{varma1994interpolation,
  title={Interpolation approximations for symmetric fork-join queues},
  author={Varma, Subir and Makowski, Armand M},
  journal={Performance Evaluation},
  volume={20},
  number={1-3},
  pages={245--265},
  year={1994},
  publisher={Elsevier}
}

@inproceedings{atar2012control,
  title={Control of fork-join networks in heavy traffic},
  author={Atar, Rami and Mandelbaum, Avishai and Zviran, Asaf},
  booktitle={2012 50th Annual Allerton Conference on Communication, Control, and Computing (Allerton)},
  pages={823--830},
  year={2012},
  organization={IEEE}
}

@article{nguyen1993processing,
  title={{Processing networks with parallel and sequential tasks: Heavy traffic analysis and Brownian limits}},
  author={Nguyen, Vi{\^e}n},
  journal={The Annals of Applied Probability},
  pages={28--55},
  year={1993},
  publisher={JSTOR}
}
@article{nguyen1994trouble,
  title={The trouble with diversity: Fork-join networks with heterogeneous customer population},
  author={Nguyen, Vi{\^e}n},
  journal={The Annals of Applied Probability},
  pages={1--25},
  year={1994},
  publisher={JSTOR}
}

@article{lu2015gaussian,
  title={Gaussian limits for a fork-join network with nonexchangeable synchronization in heavy traffic},
  author={Lu, Hongyuan and Pang, Guodong},
  journal={Mathematics of Operations Research},
  volume={41},
  number={2},
  pages={560--595},
  year={2015},
  publisher={INFORMS}
}

@article{lu2017heavy,
  title={{Heavy-traffic limits for a fork-join network in the Halfin-Whitt regime}},
  author={Lu, Hongyuan and Pang, Guodong},
  journal={Stochastic Systems},
  volume={6},
  number={2},
  pages={519--600},
  year={2017},
  publisher={INFORMS}
}

@article{lu2017heavy2,
  title={Heavy-traffic limits for an infinite-server fork-join queueing system with dependent and disruptive services},
  author={Lu, Hongyuan and Pang, Guodong},
  journal={Queueing Systems},
  volume={85},
  number={1-2},
  pages={67--115},
  year={2017},
  publisher={Springer}
}


@article{dai1992reflected,
  title={{Reflected Brownian motion in an orthant: numerical methods for steady-state analysis}},
  author={Dai, J G and Harrison, J Michael},
  journal={The Annals of Applied Probability},
  pages={65--86},
  year={1992},
  publisher={JSTOR}
}

@article{borst2004dimensioning,
  title={Dimensioning large call centers},
  author={Borst, Sem and Mandelbaum, Avi and Reiman, Martin I},
  journal={Operations Research},
  volume={52},
  number={1},
  pages={17--34},
  year={2004},
  publisher={INFORMS}
}

@article{pickands1968moment,
  title={Moment convergence of sample extremes},
  author={Pickands III, James},
  journal={The Annals of Mathematical Statistics},
  volume={39},
  number={3},
  pages={881--889},
  year={1968},
  publisher={Institute of Mathematical Statistics}
}
@article{klosterhalfen2014,
  title={Strategic safety stock placement in supply networks with static dual supply},
  author={Klosterhalfen, Steffen T and Minner, Stefan and Willems, Sean P},
  journal={Manufacturing and Service Operations Management},
  volume={16},
  number={2},
  pages={204--219},
  year={2014},
  publisher={INFORMS}
}
@article{atan2016,
  title={Inventory optimization for perishables subject to supply disruptions},
  author={Atan, Z{\"u}mb{\"u}l and Rousseau, Martine},
  journal={Optimization Letters},
  volume={10},
  number={1},
  pages={89--108},
  year={2016},
  publisher={Springer}
}


@article{nair2016provisioning,
  title={Provisioning of large-scale systems: The interplay between network effects and strategic behavior in the user base},
  author={Nair, Jayakrishnan and Wierman, Adam and Zwart, Bert},
  journal={Management Science},
  volume={62},
  number={6},
  pages={1830--1841},
  year={2016},
  publisher={INFORMS}
}

@article{gopalakrishnan2016routing,
  title={Routing and staffing when servers are strategic},
  author={Gopalakrishnan, Ragavendran and Doroudi, Sherwin and Ward, Amy R and Wierman, Adam},
  journal={Operations Research},
  volume={64},
  number={4},
  pages={1033--1050},
  year={2016},
  publisher={INFORMS}
}

@article{kumar2010exploiting,
  title={Exploiting market size in service systems},
  author={Kumar, Sunil and Randhawa, Ramandeep S},
  journal={Manufacturing \& Service Operations Management},
  volume={12},
  number={3},
  pages={511--526},
  year={2010},
  publisher={INFORMS}
}

@article{van2019economies,
  title={Economies-of-Scale in Many-Server Queueing Systems: Tutorial and Partial Review of the QED Halfin-Whitt Heavy-Traffic Regime},
  author={{\VAN{Leeuwaarden}{van}{van}} Leeuwaarden, Johan SH and Mathijsen, Britt WJ and Zwart, Bert},
  journal={SIAM Review},
  volume={61},
  number={3},
  pages={403--440},
  year={2019},
  publisher={SIAM}
}


@article{gans2003telephone,
  title={Telephone call centers: Tutorial, review, and research prospects},
  author={Gans, Noah and Koole, Ger and Mandelbaum, Avishai},
  journal={Manufacturing \& Service Operations Management},
  volume={5},
  number={2},
  pages={79--141},
  year={2003},
  publisher={INFORMS}
}

@misc{asmlreport,
  title={{ASML} Annual Report 2020},
  author={{ASML Holding N.V.}},
  howpublished={\url{https://www.asml.com/en/investors/annual-report/2020}},
  year={2021}
}

@book{piterbarg1996asymptotic,
  title={Asymptotic methods in the theory of Gaussian processes and fields},
  author={Piterbarg, Vladimir I},
  volume={148},
  year={1996},
  publisher={American Mathematical Soc.}
}

@book{mandjes2007large,
  title={Large deviations for Gaussian queues: modelling communication networks},
  author={Mandjes, Michel},
  year={2007},
  publisher={John Wiley \& Sons}
}

@article{michel1981constant,
  title={{On the constant in the nonuniform version of the Berry-Ess\'een theorem}},
  author={Michel, Reinhard},
  journal={Zeitschrift f{\"u}r Wahrscheinlichkeitstheorie und verwandte Gebiete},
  volume={55},
  number={1},
  pages={109--117},
  year={1981},
  publisher={Springer}
}

@article{bennett1962probability,
  title={Probability inequalities for the sum of independent random variables},
  author={Bennett, George},
  journal={Journal of the American Statistical Association},
  volume={57},
  number={297},
  pages={33--45},
  year={1962},
  publisher={Taylor \& Francis}
}

@article{zheng2018improved,
  title={{An improved Bennett's inequality}},
  author={Zheng, Songfeng},
  journal={Communications in Statistics-Theory and Methods},
  volume={47},
  number={17},
  pages={4152--4159},
  year={2018},
  publisher={Taylor \& Francis}
}


@incollection{brosset2022large,
  title={{Large deviations at the transition for sums of Weibull-like random variables}},
  author={Brosset, Fabien and Klein, Thierry and Lagnoux, Agn{\`e}s and Petit, Pierre},
  booktitle={S{\'e}minaire de Probabilit{\'e}s LI},
  pages={239--257},
  year={2022},
  publisher={Springer}
}

@book{billingsley2013convergence,
  title={Convergence of probability measures},
  author={Billingsley, Patrick},
  year={2013},
  publisher={John Wiley \& Sons}
}

@article{harchol2021open,
  title={Open problems in queueing theory inspired by datacenter computing},
  author={Harchol-Balter, Mor},
  journal={Queueing Systems},
  volume={97},
  number={1},
  pages={3--37},
  year={2021},
  publisher={Springer}
}



@article{raaijmakers2021fork,
  title={Fork-join and redundancy systems with heavy-tailed job sizes},
  author={Raaijmakers, Youri and Borst, Sem and Boxma, Onno},
  journal={arXiv preprint arXiv:2105.13738},
  year={2021}
}
@article{zeng2021fork,
  title={Fork and Join Queueing Networks with Heavy Tails: Scaling Dimension and Throughput Limit},
  author={Zeng, Yun and Tan, Jian and Xia, Cathy H},
  journal={Journal of the ACM (JACM)},
  volume={68},
  number={3},
  pages={1--30},
  year={2021},
  publisher={ACM New York, NY}
}

@article{xia2007scalability,
  title={Scalability of fork/join queueing networks with blocking},
  author={Xia, Cathy H and Liu, Zhen and Towsley, Don and Lelarge, Marc},
  journal={ACM SIGMETRICS Performance Evaluation Review},
  volume={35},
  number={1},
  pages={133--144},
  year={2007},
  publisher={ACM New York, NY, USA}
}

@article{resnick1973structure,
  title={The structure of extremal processes},
  author={Resnick, Sidney I and Rubinovitch, Michael},
  journal={Advances in Applied Probability},
  volume={5},
  number={2},
  pages={287--307},
  year={1973},
  publisher={Cambridge University Press}
}

@article{ballerini1985records,
  title={Records from improving populations},
  author={Ballerini, Rocco and Resnick, Sidney I},
  journal={Journal of Applied probability},
  volume={22},
  number={3},
  pages={487--502},
  year={1985},
  publisher={Cambridge University Press}
}
@article{ballerini1987records,
  title={Records in the presence of a linear trend},
  author={Ballerini, Rocco and Resnick, Sidney I},
  journal={Advances in Applied Probability},
  volume={19},
  number={4},
  pages={801--828},
  year={1987},
  publisher={Cambridge University Press}
}

@article{dwass1964extremal,
  title={Extremal processes},
  author={Dwass, Meyer},
  journal={The Annals of Mathematical Statistics},
  volume={35},
  number={4},
  pages={1718--1725},
  year={1964},
  publisher={JSTOR}
}

@article{dwass1966extremal,
  title={{Extremal processes, II}},
  author={Dwass, Meyer},
  journal={Illinois Journal of Mathematics},
  volume={10},
  number={3},
  pages={381--391},
  year={1966},
  publisher={Duke University Press}
}

@article{haji1971relation,
  title={A relation between stationary queue and waiting time distributions},
  author={Haji, Rasoul and Newell, Gordon F},
  journal={Journal of Applied Probability},
  volume={8},
  number={3},
  pages={617--620},
  year={1971},
  publisher={Cambridge University Press}
}

@book{resnick2007heavy,
  title={Heavy-tail phenomena: probabilistic and statistical modeling},
  author={Resnick, Sidney I},
  year={2007},
  publisher={Springer Science \& Business Media}
}

@inproceedings{kesten1993convergence,
  title={Convergence in distribution of lightly trimmed and untrimmed sums are equivalent},
  author={Kesten, Harry},
  booktitle={Mathematical Proceedings of the Cambridge Philosophical Society},
  volume={113},
  number={3},
  pages={615--638},
  year={1993},
  organization={Cambridge University Press}
}

@article{godreche2017record,
  title={Record statistics of a strongly correlated time series: random walks and L{\'e}vy flights},
  author={Godreche, Claude and Majumdar, Satya N and Schehr, Gregory},
  journal={Journal of Physics A: Mathematical and Theoretical},
  volume={50},
  number={33},
  pages={333001},
  year={2017},
  publisher={IOP Publishing}
}

@inproceedings{fisher1928limiting,
  title={Limiting forms of the frequency distribution of the largest or smallest member of a sample},
  author={Fisher, Ronald A and Tippett, Leonard HC},
  booktitle={Mathematical proceedings of the Cambridge philosophical society},
  volume={24},
  number={2},
  pages={180--190},
  year={1928},
  organization={Cambridge University Press}
}

@article{gnedenko1943distribution,
  title={Sur la distribution limite du terme maximum d'une serie aleatoire},
  author={Gnedenko, Boris},
  journal={Annals of mathematics},
  pages={423--453},
  year={1943},
  publisher={JSTOR}
}

@article{barndorff1963limit,
  title={On the limit behaviour of extreme order statistics},
  author={Barndorff-Nielsen, Ole},
  journal={The Annals of Mathematical Statistics},
  volume={34},
  number={3},
  pages={992--1002},
  year={1963},
  publisher={JSTOR}
}

@article{geffroy1958contributions,
  title={Contributions {\`a} la th{\'e}orie des valeurs extr{\^e}mes},
  author={Geffroy, Jean},
  journal={Publ. Inst. Statist. Univ. Paris},
  volume={7},
  pages={37--185},
  year={1958}
}

@article{fisher1969limiting,
  title={Limiting sets and convex hulls of samples from product measures},
  author={Fisher, Lloyd},
  journal={The Annals of Mathematical Statistics},
  volume={40},
  number={5},
  pages={1824--1832},
  year={1969},
  publisher={Institute of Mathematical Statistics}
}
@article{davis1988almost,
  title={{Almost sure limit sets of random samples in $\mathbb{R}^d$}},
  author={Davis, Richard A and Mulrow, Edward and Resnick, Sidney I},
  journal={Advances in applied probability},
  pages={573--599},
  year={1988},
  publisher={JSTOR}
}

@article{slepian1962one,
  title={{The one-sided barrier problem for Gaussian noise}},
  author={Slepian, David},
  journal={Bell System Technical Journal},
  volume={41},
  number={2},
  pages={463--501},
  year={1962},
  publisher={Wiley Online Library}
}

@article{bonferroni1936teoria,
  title={Teoria statistica delle classi e calcolo delle probabilita},
  author={Bonferroni, Carlo},
  journal={Pubblicazioni del R Istituto Superiore di Scienze Economiche e Commericiali di Firenze},
  volume={8},
  pages={3--62},
  year={1936}
}

@article{balkema2010meta,
  title={Meta densities and the shape of their sample clouds},
  author={Balkema, August A and Embrechts, Paul and Nolde, Natalia},
  journal={Journal of Multivariate Analysis},
  volume={101},
  number={7},
  pages={1738--1754},
  year={2010},
  publisher={Elsevier}
}


@article{anderson1997maxima,
  title={{Maxima of Poisson-like variables and related triangular arrays}},
  author={Anderson, Clive W and Coles, Stuart G and H{\"u}sler, J{\"u}rg},
  journal={The Annals of Applied Probability},
  volume={7},
  number={4},
  pages={953--971},
  year={1997},
  publisher={Institute of Mathematical Statistics}
}

@article{nagaev1969integral,
  title={{Integral limit theorems taking large deviations into account when Cram{\'e}r’s condition does not hold. I}},
  author={Nagaev, Aleksandr V},
  journal={Theory of Probability \& Its Applications},
  volume={14},
  number={1},
  pages={51--64},
  year={1969},
  publisher={SIAM}
}

@article{nagaev1969integralII,
  title={{Integral limit theorems taking large deviations into account when Cram{\'e}r’s condition does not hold. II}},
  author={Nagaev, Aleksandr V},
  journal={Theory of Probability \& Its Applications},
  volume={14},
  number={2},
  pages={193--208},
  year={1969},
  publisher={SIAM}
}

@article{nagaev1979large,
  title={Large deviations of sums of independent random variables},
  author={Nagaev, Sergey V},
  journal={The Annals of Probability},
  pages={745--789},
  year={1979},
  publisher={JSTOR}
}


@article{cramer1938nouveau,
  title={Sur un nouveau th{\'e}oreme-limite de la th{\'e}orie des probabilit{\'e}s},
  author={Cram{\'e}r, Harald},
  journal={Actual. Sci. Ind.},
  volume={736},
  pages={5--23},
  year={1938}
}

@incollection{petrov2022sums,
  title={Sums of independent random variables},
  author={Petrov, Valentin V},
  booktitle={Sums of Independent Random Variables},
  year={2022},
  publisher={De Gruyter}
}

@article{fuk1971probability,
  title={Probability inequalities for sums of independent random variables},
  author={Fuk, D Kh and Nagaev, Sergey V},
  journal={Theory of Probability \& Its Applications},
  volume={16},
  number={4},
  pages={643--660},
  year={1971},
  publisher={SIAM}
}

@article{nagaev1965some,
  title={Some limit theorems for large deviations},
  author={Nagaev, Sergey V},
  journal={Theory of Probability \& Its Applications},
  volume={10},
  number={2},
  pages={214--235},
  year={1965},
  publisher={SIAM}
}

@article{mikosch1998large,
  title={Large deviations of heavy-tailed sums with applications in insurance},
  author={Mikosch, Thomas and Nagaev, Aleksandr V},
  journal={Extremes},
  volume={1},
  number={1},
  pages={81--110},
  year={1998},
  publisher={Springer}
}

@book{dembo2009large,
  title={Large deviations techniques and applications},
  author={Dembo, Amir and Zeitouni, Ofer},
  volume={38},
  year={2009},
  publisher={Springer Science \& Business Media}
}

@book{ganesh2004big,
  title={Big queues},
  author={Ganesh, Ayalvadi J},
  year={2004},
  publisher={Springer Science \& Business Media}
}


@article{cohen1973some,
  title={Some results on regular variation for distributions in queueing and fluctuation theory},
  author={Cohen, JW},
  journal={Journal of applied probability},
  volume={10},
  number={2},
  pages={343--353},
  year={1973},
  publisher={Cambridge University Press}
}

@article{korshunov1997distribution,
  title={On distribution tail of the maximum of a random walk},
  author={Korshunov, D},
  journal={Stochastic Processes and their Applications},
  volume={72},
  number={1},
  pages={97--103},
  year={1997},
  publisher={Elsevier}
}

@article{shwartz1993induced,
  title={Induced rare events: analysis via large deviations and time reversal},
  author={Shwartz, Adam and Weiss, Alan},
  journal={Advances in Applied Probability},
  volume={25},
  number={3},
  pages={667--689},
  year={1993},
  publisher={Cambridge University Press}
}

@article{baccelli1989fork,
  title={The fork-join queue and related systems with synchronization constraints: Stochastic ordering and computable bounds},
  author={Baccelli, Fran{\c{c}}ois and Makowski, Armand M and Shwartz, Adam},
  journal={Advances in Applied Probability},
  volume={21},
  number={3},
  pages={629--660},
  year={1989},
  publisher={Cambridge University Press}
}

@article{kim1989analysis,
  title={Analysis of the fork-join queue},
  author={Kim, Cheeha and Agrawala, Ashok K},
  journal={IEEE Transactions on computers},
  volume={38},
  number={2},
  pages={250--255},
  year={1989},
  publisher={IEEE}
}

@article{duda1987performance,
  title={Performance evaluation of fork and join synchronization primitives},
  author={Duda, Andrzej and Czach{\'o}rski, Tadeusz},
  journal={Acta Informatica},
  volume={24},
  number={5},
  pages={525--553},
  year={1987},
  publisher={Springer}
}

@article{varki1999mean,
  title={Mean value technique for closed fork-join networks},
  author={Varki, Elizabeth},
  journal={ACM SIGMETRICS Performance Evaluation Review},
  volume={27},
  number={1},
  pages={103--112},
  year={1999},
  publisher={ACM New York, NY, USA}
}

@article{varki2008m,
  title={{The M/M/1 fork-join queue with variable sub-tasks}},
  author={Varki, Elizabeth and Merchant, Arif and Chen, Hui and others},
  journal={unpublished, available online},
  year={2008},
  publisher={Citeseer}
}

@inproceedings{thomasian1994approximate,
  title={{Approximate solutions for $M/G/1$ fork/join synchronization}},
  author={Thomasian, Alexander and Tantawi, Asser N},
  booktitle={Proceedings of Winter Simulation Conference},
  pages={361--368},
  year={1994},
  organization={IEEE}
}

@article{tan1996fork,
  title={A fork-join queueing model: Diffusion approximation, integral representations and asymptotics},
  author={Tan, Xiaoming and Knessl, Charles},
  journal={Queueing Systems},
  volume={22},
  number={3},
  pages={287--322},
  year={1996},
  publisher={Springer}
}

@book{bingham1989regular,
  title={Regular variation},
  author={Bingham, Nicholas H and Goldie, Charles M and Teugels, Jozef L},
  number={27},
  year={1989},
  publisher={Cambridge University Press}
}


@inproceedings{lindley1952theory,
  title={The theory of queues with a single server},
  author={Lindley, David V},
  booktitle={Mathematical Proceedings of the Cambridge Philosophical Society},
  volume={48},
  number={2},
  pages={277--289},
  year={1952},
  organization={Cambridge University Press}
}

@article{kingman1962queues,
  title={On queues in heavy traffic},
  author={Kingman, John FC},
  journal={Journal of the Royal Statistical Society: Series B (Methodological)},
  volume={24},
  number={2},
  pages={383--392},
  year={1962},
  publisher={Wiley Online Library}
}

@inproceedings{kingman1961single,
  title={The single server queue in heavy traffic},
  author={Kingman, John FC},
  booktitle={Mathematical Proceedings of the Cambridge Philosophical Society},
  volume={57},
  number={4},
  pages={902--904},
  year={1961},
  organization={Cambridge University Press}
}

@article{kendall1957some,
  title={Some problems in the theory of dams},
  author={Kendall, David G},
  journal={Journal of the Royal Statistical Society. Series B (Methodological)},
  volume={19},
  number={2},
  pages={207--233},
  year={1957},
  publisher={JSTOR}
}

@book{donsker1951invariance,
  title={An invariance principle for certain probability limit theorems},
  author={Donsker, Monroe David},
   volume={6},
  year={1951},
  publisher={Memoirs of the American Mathematical Society}
}

@article{schol2022tail,
  title={{Tail asymptotics for the delay in a Brownian fork-join queue}},
  author={Schol, Dennis and Vlasiou, Maria and Zwart, Bert},
  journal={arXiv preprint arXiv:2208.04796},
  year={2022}
}


%herhaling refs



















@article{atan2017assemble,
  title={Assemble-to-order systems: A review},
  author={Atan, Z{\"u}mb{\"u}l and Ahmadi, Taher and Stegehuis, Clara and de Kok, Ton and Adan, Ivo},
  journal={European Journal of Operational Research},
  volume={261},
  number={3},
  pages={866--879},
  year={2017},
  publisher={Elsevier}
}

@article{huh2010base,
  title={Base-stock policies in capacitated assembly systems: Convexity properties},
  author={Huh, Woonghee Tim and Janakiraman, Ganesh},
  journal={Naval Research Logistics (NRL)},
  volume={57},
  number={2},
  pages={109--118},
  year={2010},
  publisher={Wiley Online Library}
}
@article{song1999order,
  title={Order-fulfillment performance measures in an assemble-to-order system with stochastic leadtimes},
  author={Song, Jing-Sheng and Xu, Susan H and Liu, Bin},
  journal={Operations Research},
  volume={47},
  number={1},
  pages={131--149},
  year={1999},
  publisher={INFORMS}
}
@article{plambeck2008asymptotically,
  title={Asymptotically optimal control for an assemble-to-order system with capacitated component production and fixed transport costs},
  author={Plambeck, Erica L},
  journal={Operations Research},
  volume={56},
  number={5},
  pages={1158--1171},
  year={2008},
  publisher={INFORMS}
}
@article{benjaafar2006production,
  title={Production and inventory control of a single product assemble-to-order system with multiple customer classes},
  author={Benjaafar, Saif and ElHafsi, Mohsen},
  journal={Management science},
  volume={52},
  number={12},
  pages={1896--1912},
  year={2006},
  publisher={INFORMS}
}
@article{benjaafar2011optimal,
  title={Optimal control of an assembly system with multiple stages and multiple demand classes},
  author={Benjaafar, Saif and ElHafsi, Mohsen and Lee, Chung-Yee and Zhou, Weihua},
  journal={Operations Research},
  volume={59},
  number={2},
  pages={522--529},
  year={2011},
  publisher={INFORMS}
}
@article{akccay2004joint,
  title={Joint inventory replenishment and component allocation optimization in an assemble-to-order system},
  author={Ak{\c{c}}ay, Yal{\c{c}}in and Xu, Susan H},
  journal={Management Science},
  volume={50},
  number={1},
  pages={99--116},
  year={2004},
  publisher={INFORMS}
}
@article{fu2020investing,
  title={Investing in suppliers with capacity constraints in a decentralized assembly system},
  author={Fu, Hong and Li, Kai and Fu, Weizhong},
  journal={Computers \& Industrial Engineering},
  volume={142},
  pages={106332},
  year={2020},
  publisher={Elsevier}
}
@article{granot2008competition,
  title={Competition and cooperation in decentralized push and pull assembly systems},
  author={Granot, Daniel and Yin, Shuya},
  journal={Management Science},
  volume={54},
  number={4},
  pages={733--747},
  year={2008},
  publisher={INFORMS}
}
@article{guler2009coordinating,
  title={On coordinating an assembly system under random yield and random demand},
  author={G{\"u}ler, M G{\"u}ray and Bilgi{\c{c}}, Taner},
  journal={European Journal of Operational Research},
  volume={196},
  number={1},
  pages={342--350},
  year={2009},
  publisher={Elsevier}
}
@article{wang2003capacity,
  title={Capacity games in assembly systems with uncertain demand},
  author={Wang, Yunzeng and Gerchak, Yigal},
  journal={Manufacturing \& Service Operations Management},
  volume={5},
  number={3},
  pages={252--267},
  year={2003},
  publisher={INFORMS}
}
@article{zhang2006competition,
  title={Competition, cooperation, and information sharing in a two-echelon assembly system},
  author={Zhang, Fuqiang},
  journal={Manufacturing \& Service Operations Management},
  volume={8},
  number={3},
  pages={273--291},
  year={2006},
  publisher={INFORMS}
}
@article{dougru2017assemble,
  title={Assemble-to-Order Inventory Management via Stochastic Programming: Chained BOMs and the M-System},
  author={Do{\u{g}}ru, Mustafa K and Reiman, Martin I and Wang, Qiong},
  journal={Production and Operations Management},
  volume={26},
  number={3},
  pages={446--468},
  year={2017},
  publisher={Wiley Online Library}
}
@article{jaarsveld2015optimization,
  title={Optimization of industrial-scale assemble-to-order systems},
  author={van Jaarsveld, Willem and Scheller-Wolf, Alan},
  journal={INFORMS Journal on Computing},
  volume={27},
  number={3},
  pages={544--560},
  year={2015},
  publisher={INFORMS}
}
@article{elhafsi2008optimal,
  title={Optimal control of a nested-multiple-product assemble-to-order system},
  author={ElHafsi, Mohsen and Camus, Herve and Craye, Etienne},
  journal={International Journal of Production Research},
  volume={46},
  number={19},
  pages={5367--5392},
  year={2008},
  publisher={Taylor \& Francis}
}
@article{cheng2011production,
  title={Production planning and inventory allocation of a single-product assemble-to-order system with failure-prone machines},
  author={Cheng, TCE and Gao, Chunyan and Shen, Houcai},
  journal={International Journal of Production Economics},
  volume={131},
  number={2},
  pages={604--617},
  year={2011},
  publisher={Elsevier}
}



@article{coniglio2020computing,
  title={Computing a pessimistic stackelberg equilibrium with multiple followers: The mixed-pure case},
  author={Coniglio, Stefano and Gatti, Nicola and Marchesi, Alberto},
  journal={Algorithmica},
  volume={82},
  number={5},
  pages={1189--1238},
  year={2020},
  publisher={Springer}
}
@article{bacsar2002stackelberg,
  title={A Stackelberg network game with a large number of followers},
  author={Ba{\c{s}}ar, T and Srikant, R},
  journal={Journal of optimization theory and applications},
  volume={115},
  number={3},
  pages={479--490},
  year={2002},
  publisher={Springer}
}




@article{fang2017coordinated,
  title={{Coordinated multiple-relays based physical-layer security improvement: A single-leader multiple-followers Stackelberg game scheme}},
  author={Fang, He and Xu, Li and Wang, Xianbin},
  journal={IEEE transactions on information forensics and security},
  volume={13},
  number={1},
  pages={197--209},
  year={2017},
  publisher={IEEE}
}
@article{cheng2022single,
  title={Single-leader-multiple-followers Stackelberg security game with hypergame framework},
  author={Cheng, Zhaoyang and Chen, Guanpu and Hong, Yiguang},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={17},
  pages={954--969},
  year={2022},
  publisher={IEEE}
}

%herhaling refs



%herhaling refs



@article{xin2018asymptotic,
  title={Asymptotic optimality of tailored base-surge policies in dual-sourcing inventory systems},
  author={Xin, Linwei and Goldberg, David A},
  journal={Management Science},
  volume={64},
  number={1},
  pages={437--452},
  year={2018},
  publisher={INFORMS}
}

@article{goldberg2016asymptotic,
  title={Asymptotic optimality of constant-order policies for lost sales inventory models with large lead times},
  author={Goldberg, David A and Katz-Rogozhnikov, Dmitriy A and Lu, Yingdong and Sharma, Mayank and Squillante, Mark S},
  journal={Mathematics of Operations Research},
  volume={41},
  number={3},
  pages={898--913},
  year={2016},
  publisher={INFORMS}
}


@article{dougru2017,
  title={Assemble-to-Order Inventory Management via Stochastic Programming: Chained BOMs and the M-System},
  author={Do{\u{g}}ru, Mustafa K and Reiman, Martin I and Wang, Qiong},
  journal={Production and Operations Management},
  volume={26},
  number={3},
  pages={446--468},
  year={2017},
  publisher={Wiley Online Library}
}
@article{reiman2015,
  title={Asymptotically optimal inventory control for assemble-to-order systems with identical lead times},
  author={Reiman, Martin I and Wang, Qiong},
  journal={Operations Research},
  volume={63},
  number={3},
  pages={716--732},
  year={2015},
  publisher={INFORMS}
}
@article{plambeck2008,
  title={Asymptotically optimal control for an assemble-to-order system with capacitated component production and fixed transport costs},
  author={Plambeck, Erica L},
  journal={Operations Research},
  volume={56},
  number={5},
  pages={1158--1171},
  year={2008},
  publisher={INFORMS}
}
@article{plambeckward2008,
  title={Optimal control of a high-volume assemble-to-order system with maximum leadtime quotation and expediting},
  author={Plambeck, Erica L and Ward, Amy R},
  journal={Queueing Systems},
  volume={60},
  number={1},
  pages={1--69},
  year={2008},
  publisher={Springer}
}
@article{glasserman1997,
  title={Bounds and asymptotics for planning critical safety stocks},
  author={Glasserman, Paul},
  journal={Operations Research},
  volume={45},
  number={2},
  pages={244--257},
  year={1997},
  publisher={INFORMS}
}
@article{goldberg2021,
  title={A survey of recent progress in the asymptotic analysis of inventory systems},
  author={Goldberg, David A and Reiman, Martin I and Wang, Qiong},
  journal={Production and Operations Management},
  volume={30},
  number={6},
  pages={1718--1750},
  year={2021},
  publisher={Wiley Online Library}
}
@article{fu2019,
  title={Managing perishable inventory systems with product returns and remanufacturing},
  author={Fu, Ke and Gong, Xiting and Liang, Guitian},
  journal={Production and Operations Management},
  volume={28},
  number={6},
  pages={1366--1386},
  year={2019},
  publisher={Wiley Online Library}
}
@article{chaturvedi2016,
  title={Safety stock, excess capacity or diversification: Trade-offs under supply and demand uncertainty},
  author={Chaturvedi, Aadhaar and Mart{\'\i}nez-de-Alb{\'e}niz, Victor},
  journal={Production andOperations Management},
  volume={25},
  number={1},
  pages={77--95},
  year={2016},
  publisher={Wiley Online Library}
}

@misc{barrons,
  title={{ASML} Cuts Guidance in the Face of Supply-Chain Issues. The Chip Stock Is Falling},
  author={Jack Denton},
  howpublished={\url{https://www.barrons.com/articles/asml-cuts-guidance-supply-chain-issues-51634728074}},
  year={2021}
}
@article{song1998,
  title={On the order fill rate in a multi-item, base-stock inventory system},
  author={Song, Jing-Sheng},
  journal={Operations research},
  volume={46},
  number={6},
  pages={831--845},
  year={1998},
  publisher={INFORMS}
}
@article{atan2017,
  title={Assemble-to-order systems: A review},
  author={Atan, Z{\"u}mb{\"u}l and Ahmadi, Taher and Stegehuis, Clara and de Kok, Ton and Adan, Ivo},
  journal={European Journal of Operational Research},
  volume={261},
  number={3},
  pages={866--879},
  year={2017},
  publisher={Elsevier}
}
@article{lu2005,
  title={Order-based cost optimization in assemble-to-order systems},
  author={Lu, Yingdong and Song, Jing-Sheng},
  journal={Operations Research},
  volume={53},
  number={1},
  pages={151--169},
  year={2005},
  publisher={INFORMS}
}

@article{zhang2020simple,
  title={Simple policies with provable bounds for managing perishable inventory},
  author={Zhang, Hailun and Zhang, Jiheng and Zhang, Rachel Q},
  journal={Production and Operations Management},
  volume={29},
  number={11},
  pages={2637--2650},
  year={2020},
  publisher={Wiley Online Library}
}

@article{xin2016,
  title={Optimality gap of constant-order policies decays exponentially in the lead time for lost sales models},
  author={Xin, Linwei and Goldberg, David A},
  journal={Operations Research},
  volume={64},
  number={6},
  pages={1556--1565},
  year={2016},
  publisher={INFORMS}
}
@article{huh2009,
  title={Asymptotic optimality of order-up-to policies in lost sales inventory systems},
  author={Huh, Woonghee Tim and Janakiraman, Ganesh and Muckstadt, John A and Rusmevichientong, Paat},
  journal={Management Science},
  volume={55},
  number={3},
  pages={404--420},
  year={2009},
  publisher={INFORMS}
}
@article{bijvank2014,
  title={Robustness of order-up-to policies in lost-sales inventory systems},
  author={Bijvank, Marco and Huh, Woonghee Tim and Janakiraman, Ganesh and Kang, Wanmo},
  journal={Operations Research},
  volume={62},
  number={5},
  pages={1040--1047},
  year={2014},
  publisher={INFORMS}
}

@article{yao2013optimal,
  title={Optimal policy for Brownian inventory models with general convex inventory cost},
  author={Yao, Da-cheng},
  journal={Acta Mathematicae Applicatae Sinica, English Series},
  volume={29},
  number={1},
  pages={187--200},
  year={2013},
  publisher={Springer}
}


%herhaling refs

@article{amram1985multivariate,
  title={Multivariate extreme value distributions for stationary Gaussian sequences},
  author={Amram, Fred},
  journal={Journal of Multivariate Analysis},
  volume={16},
  number={2},
  pages={237--240},
  year={1985},
  publisher={Academic Press}
}
@article{abate1987transient,
  title={{Transient behavior of regulated Brownian motion, I: starting at the origin}},
  author={Abate, Joseph and Whitt, Ward},
  journal={Advances in Applied Probability},
  volume={19},
  number={3},
  pages={560--598},
  year={1987},
  publisher={Cambridge University Press}
}

@book{billingsley1968convergence,
  title={Convergence of probability measures},
  author={Billingsley, Patrick},
  year={1968},
  publisher={John Wiley \& Sons}
}


@article{sigman2011heavy,
  title={Heavy-traffic limits for nearly deterministic queues},
  author={Sigman, Karl and Whitt, Ward},
  journal={Journal of Applied Probability},
  volume={48},
  number={3},
  pages={657--678},
  year={2011},
  publisher={Cambridge University Press}
}

@article{sigman2011heavystat,
  title={Heavy-traffic limits for nearly deterministic queues: stationary distributions},
  author={Sigman, Karl and Whitt, Ward},
  journal={Queueing Systems},
  volume={69},
  number={2},
  pages={145},
  year={2011},
  publisher={Springer}
}


@article{downey1995bounds,
  title={Bounds and approximations for overheads in the time to join parallel forks},
  author={Downey, Peter J.},
  journal={ORSA Journal on Computing},
  volume={7},
  number={2},
  pages={125--139},
  year={1995},
  publisher={INFORMS}
}

@inproceedings{marin2016dynamic,
  title={Dynamic control of the join-queue lengths in saturated fork-join stations},
  author={Marin, Andrea and Rossi, Sabina},
  booktitle={International Conference on Quantitative Evaluation of Systems},
  pages={123--138},
  year={2016},
  organization={Springer}
}

@article{marin2017power,
  title={Power control in saturated fork-join queueing systems},
  author={Marin, Andrea and Rossi, Sabina},
  journal={Performance Evaluation},
  volume={116},
  pages={101--118},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{marin2018biased,
  title={Biased Processor Sharing in Fork-Join Queues},
  author={Marin, Andrea and Rossi, Sabina and Sottana, Matteo},
  booktitle={International Conference on Quantitative Evaluation of Systems},
  pages={273--288},
  year={2018},
  organization={Springer}
}


@article{stecke2009sources,
  title={Sources of supply chain disruptions, factors that breed vulnerability, and mitigating strategies},
  author={Stecke, Kathryn E and Kumar, Sanjay},
  journal={Journal of Marketing Channels},
  volume={16},
  number={3},
  pages={193--226},
  year={2009},
  publisher={Taylor \& Francis}
}

@article{luczak2006maximum,
  title={On the maximum queue length in the supermarket model},
  author={Luczak, Malwina J and McDiarmid, Colin and others},
  journal={The Annals of Probability},
  volume={34},
  number={2},
  pages={493--527},
  year={2006},
  publisher={Institute of Mathematical Statistics}
}

@misc{resilience20113rd,
  title={Supply Chain Resilience, 3rd Annual Survey},
  author={Business Continuity Institute},
  year={2011}
}

@article{norrman2004ericsson,
  title={Ericsson's proactive supply chain risk management approach after a serious sub-supplier accident},
  author={Norrman, Andreas and Jansson, Ulf},
  journal={International journal of physical distribution \& logistics management},
  volume={34},
  number={5},
  pages={434--456},
  year={2004},
  publisher={Emerald Group Publishing Limited}
}

@article{parker2015complex,
  title={Complex negative events and the diffusion of crisis: lessons from the 2010 and 2011 Icelandic volcanic ash cloud events},
  author={Parker, Charles F},
  journal={Geografiska Annaler: Series A, Physical Geography},
  volume={97},
  number={1},
  pages={97--108},
  year={2015},
  publisher={Taylor \& Francis}
}

@misc{asmlFire, title={{ASML} Integrated Report 2018}, 
author={{ASML}}, year={2018}}


@book{harrison1985brownian,
  title={Brownian motion and stochastic flow systems},
  author={Harrison, J Michael},
  year={1985},
  publisher={Wiley New York}
}


@article{dallery1994equivalence,
  title={Equivalence, reversibility, symmetry and concavity properties in fork-join queuing networks with blocking},
  author={Dallery, Yves and Liu, Zhen and Towsley, Don},
  journal={Journal of the ACM (JACM)},
  volume={41},
  number={5},
  pages={903--942},
  year={1994},
  publisher={ACM New York, NY, USA}
}

@article{dallery1997properties,
  title={Properties of fork/join queueing networks with blocking under various operating mechanisms},
  author={Dallery, Yves and Liu, Zhen and Towsley, Don},
  journal={IEEE Transactions on Robotics and Automation},
  volume={13},
  number={4},
  pages={503--518},
  year={1997},
  publisher={IEEE}
}

@article{little1961proof,
  title={A proof for the queuing formula: L= $\lambda$ W},
  author={Little, John DC},
  journal={Operations research},
  volume={9},
  number={3},
  pages={383--387},
  year={1961},
  publisher={INFORMS}
}

@book{chen2001fundamentals,
  title={Fundamentals of queueing networks: Performance, asymptotics, and optimization},
  author={Chen, Hong and Yao, David D},
  volume={4},
  year={2001},
  publisher={Springer}
}

@article{iglehart1970multipleI,
  title={{Multiple channel queues in heavy traffic. I}},
  author={Iglehart, Donald L and Whitt, Ward},
  journal={Advances in Applied Probability},
  volume={2},
  number={1},
  pages={150--177},
  year={1970},
  publisher={Cambridge University Press}
}

@article{iglehart1970multipleII,
  title={{Multiple channel queues in heavy traffic. II: Sequences, networks, and batches}},
  author={Iglehart, Donald L and Whitt, Ward},
  journal={Advances in Applied Probability},
  volume={2},
  number={2},
  pages={355--369},
  year={1970},
  publisher={Cambridge University Press}
}

@book{borovkov1984asymptotic,
  title={Asymptotic methods in queuing theory},
  author={Borovkov, Aleksandr Alekseevich},
  number={1},
  year={1984},
  publisher={John Wiley \& Sons}
}

@article{prohorov1963transient,
  title={Transient phenomena in processes of mass service},
  author={Prohorov, Yu},
  journal={Litovsk. Mat. Sb},
  volume={3},
  pages={199--205},
  year={1963}
}

@book{adler2007random,
  title={Random fields and geometry},
  author={Adler, Robert J and Taylor, Jonathan E and others},
  volume={80},
  year={2007},
  publisher={Springer}
}

@article{pickands1969upcrossing,
  title={{Upcrossing probabilities for stationary Gaussian processes}},
  author={Pickands III, James},
  journal={Transactions of the American Mathematical Society},
  volume={145},
  pages={51--73},
  year={1969}
}

@article{pickands1969asymptotic,
  title={{Asymptotic properties of the maximum in a stationary Gaussian process}},
  author={Pickands III, James},
  journal={Transactions of the American Mathematical Society},
  volume={145},
  pages={75--86},
  year={1969},
  publisher={JSTOR}
}

@article{qiu2015beyond,
  title={{Beyond the mean in fork-join queues: Efficient approximation for response-time tails}},
  author={Qiu, Zhan and P{\'e}rez, Juan F and Harrison, Peter G},
  journal={Performance Evaluation},
  volume={91},
  pages={99--116},
  year={2015},
  publisher={Elsevier}
}

@article{mena2013toward,
  title={Toward a theory of multi-tier supply chain management},
  author={Mena, Carlos and Humphries, Andrew and Choi, Thomas Y},
  journal={Journal of Supply Chain Management},
  volume={49},
  number={2},
  pages={58--77},
  year={2013},
  publisher={Wiley Online Library}
}

@misc{ahmad2010distributed,
  title={Distributed load balancer},
  author={Ahmad, Najam and Greenberg, Albert Gordon and Lahiri, Parantap and Maltz, Dave and Patel, Parveen K and Sengupta, Sudipta and Vaid, Kushagra V},
  year={2010},
  month=feb # "~11",
  publisher={Google Patents},
  note={US Patent App. 12/189,438}
}

@article{lu2011join,
  title={Join-Idle-Queue: A novel load balancing algorithm for dynamically scalable web services},
  author={Lu, Yi and Xie, Qiaomin and Kliot, Gabriel and Geller, Alan and Larus, James R and Greenberg, Albert},
  journal={Performance Evaluation},
  volume={68},
  number={11},
  pages={1056--1071},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{tirmazi2020borg,
  title={Borg: the next generation},
  author={Tirmazi, Muhammad and Barker, Adam and Deng, Nan and Haque, Md E and Qin, Zhijing Gene and Hand, Steven and Harchol-Balter, Mor and Wilkes, John},
  booktitle={Proceedings of the fifteenth European conference on computer systems},
  pages={1--14},
  year={2020}
}

@article{wang2019delay,
  title={Delay asymptotics and bounds for multitask parallel jobs},
  author={Wang, Weina and Harchol-Balter, Mor and Jiang, Haotian and Scheller-Wolf, Alan and Srikant, Rayadurgam},
  journal={Queueing Systems},
  volume={91},
  number={3},
  pages={207--239},
  year={2019},
  publisher={Springer}
}

@book{nair2022fundamentals,
  title={{The fundamentals of heavy tails: Properties, emergence, and estimation}},
  author={Nair, Jayakrishnan and Wierman, Adam and Zwart, Bert},
  volume={53},
  year={2022},
  publisher={Cambridge University Press}
}

@article{adamchik1998some,
  title={{Some series of the zeta and related functions}},
  author={Adamchik, Victor S and Srivastava, HM},
  journal={Analysis},
  volume={18},
  number={2},
  pages={131--144},
  year={1998},
  publisher={Oldenbourg Wissenschaftsverlag}
}
